Incoherence of Partial-Component Sampling in multidimensional NMR

In NMR spectroscopy, undersampling in the indirect dimensions causes reconstruction artifacts whose size can be bounded using the so-called {\it coherence}. In experiments with multiple indirect dimensions, new undersampling approaches were recently proposed: random phase detection (RPD) \cite{Maciejewski11} and its generalization, partial component sampling (PCS) \cite{Schuyler13}. The new approaches are fully aware of the fact that high-dimensional experiments generate hypercomplex-valued free induction decays; they randomly acquire only certain low-dimensional components of each high-dimensional hypercomplex entry. We provide a classification of various hypercomplex-aware undersampling schemes, and define a hypercomplex-aware coherence appropriate for such undersampling schemes; we then use it to quantify undersampling artifacts of RPD and various PCS schemes.

==> ReproduceMe/analysis/Coherence_NUSvsPCS/Table_MethodEquiDist_FOURIER_delta2.5e-01.tex <==
% latex table generated in R 3.2.2 by xtable 1.8-0 package
% Fri Dec 11 18:43:46 2015
\begin{table}[ht]
\centering
\caption{mean, standard deviation and KS statistic for coherence of NUS, FDPCS, and PCS. Here the ensemble is Fourier, $\delta = 0.25$ and nMonte = 510. The experiments are conducted for approach A2, and scheme S4 on a 2D square indel lattice of size N=20,40,60,80, and 100'. Corresponding p-vaues are shown in parentheses.} 
\label{MethodEquiDist_delta2.5e-01}
\begin{tabular}{rlllll}
  \hline
 & 20 & 40 & 60 & 80 & 100 \\ 
  \hline
D(NUS,PCS) & 0.471 (0.000) & 0.262 (0.000) & 0.105 (0.199) & 0.067 (0.739) & 0.137 (0.000) \\ 
  D(NUS,FDPCS) & 0.671 (0.000) & 0.448 (0.000) & 0.233 (0.000) & 0.167 (0.006) & 0.139 (0.000) \\ 
   \hline
\end{tabular}
\end{table}


==> ReproduceMe/analysis/Coherence_NUSvsPCS/Table_MethodEquiDist_FOURIER_delta5e-01.tex <==
% latex table generated in R 3.2.2 by xtable 1.8-0 package
% Fri Dec 11 18:43:46 2015
\begin{table}[ht]
\centering
\caption{mean, standard deviation and KS statistic for coherence of NUS, FDPCS, and PCS. Here the ensemble is Fourier, $\delta = 0.50$ and nMonte = 510. The experiments are conducted for approach A2, and scheme S4 on a 2D square indel lattice of size N=20,40,60,80, and 100'. Corresponding p-vaues are shown in parentheses.} 
\label{MethodEquiDist_delta5e-01}
\begin{tabular}{rlllll}
  \hline
 & 20 & 40 & 60 & 80 & 100 \\ 
  \hline
D(NUS,PCS) & 0.505 (0.000) & 0.181 (0.002) & 0.086 (0.423) & 0.081 (0.497) & 0.186 (0.000) \\ 
  D(NUS,FDPCS) & 0.610 (0.000) & 0.319 (0.000) & 0.210 (0.000) & 0.110 (0.161) & 0.078 (0.087) \\ 
   \hline
\end{tabular}
\end{table}


==> ReproduceMe/analysis/Coherence_NUSvsPCS/Table_MethodEquiMedian_FOURIER_delta2.5e-01.tex <==
% latex table generated in R 3.2.2 by xtable 1.8-0 package
% Fri Dec 11 20:14:12 2015
\begin{table}[ht]
\centering
\caption{median, standard deviation and z-score of median difference for NUS, FDPCS, and PCS coherence. Here the ensemble is Fourier, $\delta = 0.25$ and nMonte = 510. The experiments are conducted for approach A2, and scheme S4 on a 2D square indel lattice of size N=20,40,60,80, and 100'. Standard deviations are shown in parentheses.} 
\label{MethodEquiMean_delta2.5e-01}
\begin{tabular}{rlllll}
  \hline
 & 20 & 40 & 60 & 80 & 100 \\ 
  \hline
NUS & 0.209 (1.60e-03) & 0.115 (5.79e-04) & 0.082 (5.13e-04) & 0.063 (4.26e-04) & 0.051 (1.98e-04) \\ 
  PCS & 0.237 (1.74e-03) & 0.123 (9.70e-04) & 0.084 (6.08e-04) & 0.064 (4.79e-04) & 0.051 (1.65e-04) \\ 
  FDPCS & 0.256 (2.38e-03) & 0.127 (8.89e-04) & 0.085 (3.87e-04) & 0.065 (3.78e-04) & 0.053 (1.90e-04) \\ 
  Z(NUS,PCS) & -11.653 & -6.448 & -2.337 & -0.469 & 1.133 \\ 
  Z(NUS,FDPCS) & -16.199 & -11.163 & -5.298 & -2.215 & -5.627 \\ 
   \hline
\end{tabular}
\end{table}


==> ReproduceMe/analysis/Coherence_NUSvsPCS/Table_MethodEquiMedian_FOURIER_delta5e-01.tex <==
% latex table generated in R 3.2.2 by xtable 1.8-0 package
% Fri Dec 11 20:14:13 2015
\begin{table}[ht]
\centering
\caption{median, standard deviation and z-score of median difference for NUS, FDPCS, and PCS coherence. Here the ensemble is Fourier, $\delta = 0.50$ and nMonte = 510. The experiments are conducted for approach A2, and scheme S4 on a 2D square indel lattice of size N=20,40,60,80, and 100'. Standard deviations are shown in parentheses.} 
\label{MethodEquiMean_delta5e-01}
\begin{tabular}{rlllll}
  \hline
 & 20 & 40 & 60 & 80 & 100 \\ 
  \hline
NUS & 0.118 (9.29e-04) & 0.067 (4.20e-04) & 0.047 (2.70e-04) & 0.036 (1.90e-04) & 0.030 (1.06e-04) \\ 
  PCS & 0.134 (8.04e-04) & 0.070 (6.21e-04) & 0.048 (2.62e-04) & 0.036 (2.34e-04) & 0.030 (9.17e-05) \\ 
  FDPCS & 0.140 (1.01e-03) & 0.072 (7.60e-04) & 0.049 (2.57e-04) & 0.037 (1.75e-04) & 0.030 (8.53e-05) \\ 
  Z(NUS,PCS) & -13.2 & -4.43 & -2.015 & -0.607 & 3.011 \\ 
  Z(NUS,FDPCS) & -15.613 & -5.914 & -5.431 & -3.418 & -0.875 \\ 
   \hline
\end{tabular}
\end{table}

